Technology developments for LHCb Upgrade II

A major LHCb detector upgrade will be installed during long shutdown~4 (LS4) of the CERN Large Hadron Collider. The experiment will operate at a maximum luminosity of up to $1.5\times 10^{34}\mathrm{cm}^{-2}\mathrm{s}^{-1}$, with acceptance covering a pseudorapidity range close to the beamline. The detector will therefore experience extremely high particle fluences. In order to carry out the LHCb physics programme, technologies are being developed that can withstand the high rates and associated radiation damage while also providing excellent resolution in both space and time. The amount of data to be processed in the online computing and trigger system is also unprecedented. In this document, the technology developments that are necessary to realise this programme are summarised.

==> Infrastructure/Infrastructure.tex <==
\subsection{Infrastructure}
\label{sec:Subdetectors:Infrastructure}

\subsubsection*{Cooling}
Based on the preliminary sets of specifications (Table~\ref{Tab:CoolingSpecs}), the detector cooling requirements of the Upgrade~II experiment can be covered by three different technologies/coolants:
\begin{itemize}
  \item
  a liquid nitrogen (LN2) cryogenic cooling system for the silicon photomultipliers of the RICH and MT-SciFi detectors, and also possibly for the TORCH detector,
  \item
  a two-phase accumulator-controlled (2PACL) CO$_{2}$ cooling system for the VELO, UP and MT-CMOS silicon pixel detectors,
  \item
  water cooling for the front-end electronics of the MT-SciFi and RICH detectors, and other systems that do not require low-temperature cooling.
\end{itemize}
For the LN2 system, a conceptual design study, including the integration of the different components (Turbo-Brayton subcooler, phase separator, pumps, valve boxes, distribution boxes, cryogenic transfer lines, surface dewar), is being performed in collaboration with the CERN TE-CRG group.

The expected power dissipation of the Upgrade~II silicon detectors will exceed significantly the capacity of the existing VELO/UT evaporative CO$_{2}$ cooling plants. For the ATLAS and CMS Phase~2 Upgrades, new CO$_{2}$ systems are currently being constructed which, thanks to their modular design, should be straightforward to adapt for LHCb. In addition to the secondary CO$_{2}$ cooling plants, a new primary refrigeration system will also be needed which, following the ATLAS/CMS Phase~2 approach, would also be based on CO$_{2}$ (R744). 
This will require a new technical building on the surface of Point 8 to host the primary system, and new CO$_{2}$ transfer lines between surface and underground. 

In addition to the final detector cooling systems, smaller scale versions and prototypes will need to be constructed for R\&D and detector assembly.

%Refurbishment of the D1 and D2 counting rooms. 
%Mixed water. Use demin. water instead?

The capacity of the existing ventilation system is expected to be sufficient for Upgrade~II. However, local modifications of air ducts are likely to be needed, \eg\ due to the new cryogenic and CO$_{2}$ detector cooling systems. The ventilation of the UX85 cavern currently uses 100\% fresh air, which should be reviewed in terms of energy efficiency. 

%In step with the more stringent cooling requirements, the capacity of the dry gas flushing systems will need to be expanded.
%The existing gas systems will need to be refurbished and a new gas system for the Muon $\upmu$-RWELL detectors will need to be added.

\begin{table}[!b]
  \centering
  \caption{Preliminary detector cooling requirements in the Baseline scenario.}
  \label{Tab:CoolingSpecs}
    \renewcommand{\arraystretch}{1.1}
  \begin{tabular}{l r r}
%    \toprule
\hline
    System & \multicolumn{1}{c}{Coolant temperature [$^{\circ}$C]} & \multicolumn{1}{c}{Power [kW]} \\
    \hline
    VELO     & $< -40$ &  4 \\
    UP       &   $-30$ & 26 \\
    MT-CMOS  &   $-30$ & 54 \\
    MT-SciFi &  $-190$ &  4 \\
    RICH     & $-190$ &  10 \\
%    \bottomrule
\hline
  \end{tabular}
\end{table}
\subsubsection*{Magnet}
Potential failure modes related to mechanical fatigue and radiation-induced degradation have been reviewed and no show-stoppers that would prevent operating the existing normal-conducting dipole magnet throughout Run 5 and Run 6 have been identified \cite{EDMS3091606}.
In LS3, the EPDM hoses at the water cooling inlets and outlets of the coils will be replaced preventively. The magnet safety system (MSS) is planned to be upgraded in LS4.

\subsubsection*{Safety and radiation protection}
The Upgrade~II detector and its services (in particular the detector cooling systems) are likely to introduce hazard scenarios that will require the installation of additional safety systems, \eg\ oxygen deficiency or CO$_{2}$ detection.
%
The hardware components of the Detector Safety System (DSS), operating uninterruptedly since 2004, have exceeded their service life and will be replaced during LS3.
The SNIFFER system is also facing obsolescence and will be replaced in LS3 by off-the-shelf aspirating smoke detectors. 
The fire detection in the electronic racks should also be reviewed, and alternatives to the existing CO$_{2}$ based fire suppression system should be investigated. 

In view of the increased radiological risk due to the increase in luminosity in Upgrade~II, a quantitative assessment of fire-related risks is planned to be performed within the context of the CERN FIRIA (Fire-Induced Radiological Integrated Assessment) project. 

Radiation simulations will be crucial to guide the detector design, prepare procedures for dismantling, modification of components and installation, and determine the radioactive zoning of the cavern for LS4. 
The detectors shall be designed not only to withstand the harsh environment in terms of hadron fluence and total ionising dose accumulated over the Upgrade~II lifetime, but also with a view to reducing exposure to radiation during maintenance and repair interventions.

\subsubsection*{Power distribution}
The two 1.25\,MVA transformers located in the UX85 cavern are expected to provide sufficient margin to supply the required power for the detector and associated services in Upgrade~II.
Modifications to the electrical distribution downstream of the transformers will be needed in LS4 to meet the requirements of the 
upgraded detector and services.

The 400\,V distribution boards feeding the racks in the D1, D2, and D3 counting rooms (Fig.~\ref{Fig:LayoutUX85}) date from LEP times and are planned to be replaced during LS3.
%
Additionally, most of the low-voltage and high-voltage supplies will be 25 years old by the start of LS4 and will therefore need replacement. LHCb is currently studying the feasibility of using new supplies developed for the ATLAS/CMS Phase-2 upgrades. Results are encouraging and this would offer the best solution both technically and financially. This would also allow preparatory work on the required infrastructure to start already in LS3.

If the detector needs to be kept cold at all times and cooling, vacuum, 
and dry gas systems need to be running uninterruptedly, a diesel 
generator set dedicated to the experiment will need to be installed. 

\subsubsection*{Computing facilities}
As a baseline, it is assume that, due to length limitations of the optical link, part of the event-builder system for Upgrade~II will be located in the UX85 cavern. 
This requires a refurbishment of the D1 and/or D2 counting rooms, which is planned for LS3. 
\begin{figure}[!tb]
  \centering
  \includegraphics[width=0.7\textwidth]{Infrastructure/Infrastructure-figs/LayoutUX85.pdf}
  \caption{Layout of the LHCb cavern, indicating the location of the D1--D3 counting rooms and the shielding wall separating UX85A and UX85B.}
  \label{Fig:LayoutUX85}
\end{figure}
%Optical fibres linking the readout system underground to the modular data centre on the surface will need to be installed.

By the end of Run~4, the modular data centre on the surface will have been in operation for more than ten years and will require a partial refurbishment.
This will include replacement of the air-handling units.

\subsubsection*{Buildings}
During the Upgrade~I construction phase, the existing LHCb facilities at Point 8, \ie\ the SXL8 hall (which includes a $40\m^{2}$ cleanroom) and the so-called ``grey room'' in the SX8 hall, were fully utilized for the assembly and pre-commissioning of the UT and SciFi detectors.
For the construction of the Upgrade~II tracking detectors additional space will be needed, which requires the construction of a new building at Point 8 or the use of existing facilities elsewhere at CERN (provided that they become available by the first year of Run~4). 
Space on the surface will also be required for the modification of the bridge.
In the scenarios that foresee a new RICH2 vessel, a clean space of at least the same size as the SX8 ``grey room'' will be needed. 
Suitable laboratory and temporary storage space at Point 8 will also be required for the calorimeter modules and muon chambers that need to be reworked and modified during LS4. In addition, the existing radioactive buffer storage will need to be consolidated to ensure efficient dismantling of the Upgrade~I systems. 

\subsubsection*{Cost}
Table~\ref{Tab:CostInfrastructure} shows the cost estimate for common infrastructure in the Baseline scenario. 
The first category (``common electronics'') comprises a shared pool of spare PCIe400 readout boards, low-voltage supplies and electronics components (DC-DC converters, lpGBT, VTRX+), as well as the refurbishment of electronics racks and control infrastructure. 
Detector cooling is one of the main cost drivers in the second category (``General infrastructure''). The associated costs comprise a new primary CO$_{2}$ (R744) cooling system (including a new technical building and associated services), storage tanks and backup systems, support structures, installation of transfer lines, adaptation of ventilation ducts and water cooling circuits, electrical connections, new safety systems (oxygen deficiency hazard and CO$_{2}$ detection), and auxiliary services (\eg\ dry air supply).
In addition to a new technical building, the item ``civil engineering and buildings'' includes a new assembly hall as well as additional storage and buffer space, assuming a similar sharing of costs between CERN as host laboratory and collaboration funds as for the ATLAS and CMS Phase-2 upgrades. 
The category ``Data centre facilities'' includes the refurbishment of the D1 and D2 counting rooms but not the upgrade of the modular data centre at the surface of Point 8.

For Middle and Low scenarios, a cost reduction of $\sim 8\%$ and $\sim 14 \%$ with respect to
Baseline is achieved, respectively, due to the reduced needs of the detector. 
\begin{table}[!tb]
  \centering
  \caption{Cost estimate for common infrastructure in Baseline scenario.}
  \label{Tab:CostInfrastructure}
    \renewcommand{\arraystretch}{1.1}
  \begin{tabular}{l l r r}
    \hline
  &  & \multicolumn{2}{c}{Cost [kCHF]} \\
    \hline
\multicolumn{2}{l}{Common electronics}                &  1635 & \\
                       & Readout boards               &       & 441 \\
                       & Power supplies               &       &  238 \\
                       & Racks, monitoring            &       &  300 \\
                       & Common spare components          &       &  656 \\
\multicolumn{2}{l}{General infrastructure}           & 12328 \\
                       & Civil engineering, buildings &       & 1540 \\
                       & Cooling, ventilation, gas    &       & 4010 \\
                       & Assembly                     &       &  600 \\
                       & Installation                 &       &  1648 \\
                       & Access and support structures          &       &  600 \\
                       & Electrical power             &       &  1150 \\
                       & Radiation shielding          &       &  300 \\
                       & Survey                       &       &  460 \\
                       & Long-distance cabling        &       &  600 \\
                       & Safety                       &       & 1420 \\
\multicolumn{2}{l}{Data centre facilities}            &  500 \\
                       & Refurbishment UX85           &       & 500 \\
    \hline
                       &                              & 14463 &  \\ 
    \hline
  \end{tabular}
\end{table}

==> Infrastructure/LS4Schedule.tex <==
\definecolor{DarkGreen}{RGB}{0,100,0}
\definecolor{DarkPlum}{RGB}{144,80,64}
\definecolor{DarkGrey}{RGB}{160,160,160}
\definecolor{Gold}{RGB}{255,215,0}
\definecolor{SkyBlue}{RGB}{135,206,235}

\begin{tikzpicture}

\newganttchartelement{outbar}{
  outbar/.style={draw=none,fill=DarkGreen,shape=rounded rectangle,inner sep=0pt},
  outbar label font=\footnotesize
}
\newganttchartelement{inbar}{
  inbar/.style={draw=none,fill=DarkPlum,shape=rounded rectangle,inner sep=0pt},
  inbar label font=\footnotesize
}
\newganttchartelement{outinbar}{
  outinbar/.style={draw=none,left color=DarkGreen,right color=DarkPlum,shape=rounded rectangle,inner sep=0pt},
  outinbar label font=\footnotesize
}
\newganttchartelement{bpbar}{
  bpbar/.style={draw=none,fill=DarkGrey,shape=rounded rectangle,inner sep=0pt},
  %bpbar/.style={draw=none,fill=DarkGrey},
  bpbar label font=\footnotesize
}

\begin{ganttchart}[
    expand chart=1.5\textwidth,
    x unit=1mm,
    y unit title=5mm,
    y unit chart=5mm,
    %inline,
    canvas/.append style={fill=none,draw=none},
    title/.style={draw=none,fill=none},
    title height=1,
    title label font=\footnotesize,
    bar label font=\footnotesize,
    bar/.append style={draw=none,fill=Gold,rounded corners=3pt},
    milestone/.append style={fill=red,shape=diamond},
    milestone label font=\footnotesize,
    time slot format=isodate,
    %time slot unit=month,
    %link/.style={-latex, line width=1.5pt, linkred},
  ]{2032-12-01}{2035-02-28}
  \gantttitlecalendar{year,month} \\
  %\ganttbar[bar inline label node/.style=above]{Open detectors}{2033-01-01}{2033-01-15} 
  \ganttoutinbar[name=svc]{Remove and install services}{2032-12-01}{2033-12-31} \\
  \ganttbpbar[name=bpout]{Remove beam pipe (2 -- 4)}{2033-01-15}{2033-02-28} \\
  \ganttoutbar[name=sfout]{Remove SciFi and bridge}{2033-03-01}{2033-05-01} \\
  \ganttoutbar[name=r2out]{Remove RICH2}{2033-05-01}{2033-06-01} \\
  \ganttinbar[name=ms]{Install magnet stations}{2033-06-01}{2033-08-01} \\
  \ganttinbar[name=r2in]{Install RICH2/TORCH}{2033-07-01}{2034-04-01} \\
  \ganttinbar[name=brin]{Install bridge}{2033-08-01}{2033-10-01} \\
  \ganttinbar[name=mtin]{Install MT}{2033-10-01}{2034-04-01} 
  \ganttinbar[name=mtina]{}{2034-06-01}{2034-09-01} \\
  \ganttoutbar[name=calout]{Dismantle ECAL}{2033-03-01}{2033-07-01} \\
  \ganttbar[bar/.append style={shape=ellipse, fill=SkyBlue}]{Modify ECAL modules}{2033-04-15}{2034-02-01} \\
  \ganttinbar[name=calin]{Install PicoCal}{2033-10-01}{2034-04-01} \\
  \ganttoutinbar[name=mu]{Replace muon chambers}{2033-01-01}{2034-09-01} \\
  \ganttoutbar[name=utout]{Remove UT}{2033-01-01}{2033-03-01} \\
  \ganttbpbar[name=bp1out]{Remove RICH1 optics and beam pipe 1}{2033-03-01}{2033-04-01} \\
  \ganttoutbar[name=r1out]{Remove RICH1 mechanics}{2033-04-01}{2033-05-01} \\
  \ganttoutbar[name=veout]{Remove VELO}{2033-05-01}{2033-07-01} \\

  \ganttinbar[name=rfin]{Install VELO vessel}{2033-08-01}{2033-10-01} \\
  \ganttinbar[name=r1in1]{Install RICH1 mechanics}{2033-10-01}{2033-11-15} \\
  \ganttbpbar[name=bp1in]{Install beam pipe 1}{2033-11-15}{2033-12-01} \\
  \ganttinbar[name=utin]{Install UT}{2033-12-01}{2034-04-01} \\
  \ganttbpbar[name=bpin]{Install beam pipe (2 -- 4), bakeout}{2034-04-01}{2034-06-01} \\
  \ganttinbar[name=r1in2]{Install RICH1 optics and photon detectors}{2034-06-01}{2034-07-15} \\
  \ganttinbar[name=vein]{Install VELO modules}{2034-07-15}{2034-09-01} \\
  \ganttbar[name=co]{Global commissioning}{2034-09-01}{2035-03-01} 
  %\ganttbar[name=co1,inline=true,bar label inline node/.style=below]{$\neq$ margin for installation}{2034-09-01}{2035-03-01}
  %\ganttvrule[vrule/.append style={thin,dashed}]{}{2034-04-01}
\end{ganttchart}
\node[anchor=north east,font=\footnotesize] at (-1,0) {Baseline scenario};
\end{tikzpicture}


==> Infrastructure/LS4ScheduleFrugal.tex <==

\begin{tikzpicture}
\newganttchartelement{outbar}{
  outbar/.style={draw=none,fill=DarkGreen,shape=rounded rectangle,inner sep=0pt},
  outbar label font=\footnotesize
}
\newganttchartelement{inbar}{
  inbar/.style={draw=none,fill=DarkPlum,shape=rounded rectangle,inner sep=0pt},
  inbar label font=\footnotesize
}
\newganttchartelement{outinbar}{
  outinbar/.style={draw=none,left color=DarkGreen,right color=DarkPlum,shape=rounded rectangle,inner sep=0pt},
  outinbar label font=\footnotesize
}
\newganttchartelement{bpbar}{
  bpbar/.style={draw=none,fill=DarkGrey,shape=rounded rectangle,inner sep=0pt},
  %bpbar/.style={draw=none,fill=DarkGrey},
  bpbar label font=\footnotesize
}

\begin{ganttchart}[
    expand chart=\textwidth,
    x unit=0.1cm,
    y unit title=3.5mm,
    y unit chart=3.5mm,
    %inline,
    canvas/.append style={fill=none,draw=none},
    title/.style={draw=none,fill=none},
    title height=1,
    title label font=\footnotesize,
    bar label font=\footnotesize,
    bar/.append style={draw=none,fill=Gold,rounded corners=3pt},
    milestone/.append style={fill=red,shape=diamond},
    milestone label font=\footnotesize,
    time slot format=isodate,
    %time slot unit=month,
    %link/.style={-latex, line width=1.5pt, linkred},
  ]{2032-12-01}{2035-02-28}
  \gantttitlecalendar{year,month} \\
  %\ganttbar[bar inline label node/.style=above]{Open detectors}{2033-01-01}{2033-01-15} 
  \ganttoutinbar[name=svc]{Remove and install services}{2032-12-01}{2033-12-31} \\
  \ganttbpbar[name=bpout]{Remove beam pipe (2 -- 4)}{2033-01-15}{2033-02-28} \\
  \ganttoutbar[name=sfout]{Remove SciFi and bridge}{2033-03-01}{2033-05-01} \\
  \ganttoutinbar[name=r2]{Upgrade RICH2 in situ}{2033-05-01}{2034-04-01} \\
  \ganttinbar[name=brin]{Install bridge}{2033-07-01}{2033-09-01} \\
  \ganttinbar[name=mtin]{Install MT}{2033-09-01}{2034-04-01} 
  \ganttinbar[name=mtina]{}{2034-06-01}{2034-09-01} \\
  \ganttoutbar[name=calout]{Dismantle ECAL}{2033-03-01}{2033-07-01} \\
  \ganttbar[bar/.append style={shape=ellipse, fill=SkyBlue}]{Modify ECAL modules}{2033-04-15}{2034-02-01} \\
  \ganttinbar[name=calin]{Install PicoCal}{2033-10-01}{2034-04-01} \\
  \ganttoutinbar[name=mu]{Replace muon chambers}{2033-01-01}{2034-09-01} \\
  \ganttoutbar[name=utout]{Remove UT}{2033-01-01}{2033-03-01} \\
  \ganttbpbar[name=bp1out]{Remove RICH1 optics and beam pipe 1}{2033-03-01}{2033-04-01} \\
  \ganttoutbar[name=r1out]{Remove RICH1 mechanics}{2033-04-01}{2033-05-01} \\
  \ganttoutbar[name=veout]{Remove VELO}{2033-05-01}{2033-07-01} \\

  \ganttinbar[name=rfin]{Install VELO vessel}{2033-08-01}{2033-10-01} \\
  \ganttinbar[name=r1in1]{Install RICH1 mechanics}{2033-10-01}{2033-11-15} \\
  \ganttbpbar[name=bp1in]{Install beam pipe 1}{2033-11-15}{2033-12-01} \\
  \ganttinbar[name=utin]{Install UT}{2033-12-01}{2034-04-01} \\
  \ganttbpbar[name=bpin]{Install beam pipe (2 -- 4), bakeout}{2034-04-01}{2034-06-01} \\
  \ganttinbar[name=r1in2]{Install RICH1 optics and photon detectors}{2034-06-01}{2034-07-15} \\
  \ganttinbar[name=vein]{Install VELO modules}{2034-07-15}{2034-09-01} \\
  \ganttbar[name=co]{Global commissioning}{2034-09-01}{2035-03-01} 
  %\ganttbar[name=co1,inline=true,bar label inline node/.style=below]{$\neq$ margin for installation}{2034-09-01}{2035-03-01}
  %\ganttvrule[vrule/.append style={thin,dashed}]{}{2034-04-01}
  %\ganttmilestone{Start of commissioning}{2034-09-01}
\end{ganttchart}
\node[anchor=north east,font=\footnotesize] at (-1,0) {Frugal scenario};
\end{tikzpicture}


==> Online/Online.tex <==
\subsection{Online}
\label{sec:Subdetectors:Online}
%\textcolor{blue}{Editing team members responsible: Vava}

The Online system, as a physical infrastructure, consists of several parts: the controls network, the server infrastructure for the experiment control system, and the timing and fast control system. The Online system also encompasses general infrastructure such as the workstations and network for the control room and the various assembly halls. All these aforementioned systems are (largely) independent of the exact number of readout-channels or subdetectors. 

There is another important part of the Online system, which does scale with the number of readout-channels and with the total amount of data. 
The number of readout-servers and ECS front-end servers scales with the number of optical links for DAQ and controls. The size of the event-building network scales, to first order, with the gross (\ie\ including headers, protocols, \etc) aggregate of data from the detector. 

For a given amount of total raw data the amount of links has a lower limit because of the maximum throughput capacity of a lpGBT link of about 10~Gbit/s. However geometrical, organisational and other considerations in the design of the front-end electronics can and do increase the number of DAQ and ECS links significantly. By under-using the links their number and the cost in the DAQ/ECS-front-end part of the Online system are increased.

If one assumes that for a given schema for the subdetector readouts the number of links scales linearly with the luminosity --- which is a reasonable assumption for the DAQ\footnote{Not necessarily for the ECS links, but these are a fairly small fraction of the overall Online system cost.} --- and if the granularity of the detector also follows the instantaneous luminosity, then the total variable cost of the Online system will also scale linearly with the luminosity.

The Online system costs for the Baseline and Middle scenarios are given in Table~\ref{tab:online-cost-u2}, which also indicates the number of available GPU slots in the event-builder servers. As the number of servers decreases the number of available slots also decreases. In all these numbers rounding effects and partitioning considerations\footnote{Hardware from different subdetectors is not mixed. This has been found to be very important for the simplicity of operations and in particular for the commissioning of the subdetectors.} have been ignored.
With respect to Middle scenario, a further 5\% cost reduction is achieved for Low,  which is achieved mainly by removal of TORCH and Magnet Stations.

\begin{table}[!b]
    \centering
        \caption{Cost estimate of Online system for Baseline and  Middle scenarios. The peak luminosity and the number of available GPU slots is also reported for each scenario. Fixed cost refers to the infrastructure components which are luminosity-independent.}
    \label{tab:online-cost-u2}
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{lrr}
       \hline
                                   & Baseline  & Middle \\
     ${\cal L}_{\rm peak}$  ($10^{34}\cm^{-2}\sec^{-1}$) & $1.5$ & $1.0$  \\
           Available GPU slots & 840  & 560 \\
       \hline 
%       Fixed cost [kCHF]   & 3,00   & 3,000  &	3,000 \\
%       Variable cost [kCHF] & 8,800  & 7 ,627	& 5,867 \\
                                &  (kCHF)  &  (kCHF) \\
              Fixed cost        &  4800   & 	4800 \\
       Variable cost            &  7000   &   4667 \\ \hline
       Total Online             & 11800   & 	9467 \\
       \hline
    \end{tabular}
\end{table}

\begin{comment}
\begin{table}[!b]
    \centering
        \caption{Cost estimate of Online system for Baseline, Middle~(1.3) and Middle~(1.0) (equivalent to Low) scenarios. The peak luminosity and the number of available GPU slots is also reported for each sceanrio. Fixed cost refers to the infrastructure components which are luminosity-independent.}
    \label{tab:online-cost-u2}
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{lrrr}
       \hline
                                   & Baseline & Middle~(1.3) & Middle~(1.0) \\
     ${\cal L}_{\rm peak}$  ($10^{34}\cm^{-2}\sec^{-1}$) & $1.5$ & $1.3$ & $1.0$  \\
           Available GPU slots & 840 & 728 & 560 \\
       \hline 
%       Fixed cost [kCHF]   & 3,00   & 3,000  &	3,000 \\
%       Variable cost [kCHF] & 8,800  & 7 ,627	& 5,867 \\
                                &  (kCHF)  & (kCHF) & (kCHF) \\
              Fixed cost        &  4800   & 4800  &	4800 \\
       Variable cost            &  7000   & 6067	&  4667 \\
       Total Online             & 11800   & 10867 &	9467 \\
       \hline
    \end{tabular}
\end{table}
\end{comment}


Because most the variable costs are driven by I/O and not computational power, the price-compression factor is different than that used for the HLT. It is also more difficult to estimate, because the evolution in I/O speed proceeds in large jumps, not in ``quasi-continuous'' increments. While higher speed decreases the cost per unit of data transported, it however  requires more and more sophisticated materials in the server hardware, which tends to drive cost up. The quoted numbers are based on reasonable assumptions on the price compression based on long-term experience with the Online system. %We have tried to make some reasonable assumptions on the price compression based on long-term experience in the Online team. %and we do not think it wise to assume any beyond that. 

==> figs/LS4Schedule.tex <==
\definecolor{DarkGreen}{RGB}{0,100,0}
\definecolor{DarkPlum}{RGB}{144,80,64}
\definecolor{DarkGrey}{RGB}{160,160,160}
\definecolor{Gold}{RGB}{255,215,0}
\definecolor{SkyBlue}{RGB}{135,206,235}

\begin{tikzpicture}

\newganttchartelement{outbar}{
  outbar/.style={draw=none,fill=DarkGreen,shape=rounded rectangle,inner sep=0pt},
  outbar label font=\footnotesize
}
\newganttchartelement{inbar}{
  inbar/.style={draw=none,fill=DarkPlum,shape=rounded rectangle,inner sep=0pt},
  inbar label font=\footnotesize
}
\newganttchartelement{outinbar}{
  outinbar/.style={draw=none,left color=DarkGreen,right color=DarkPlum,shape=rounded rectangle,inner sep=0pt},
  outinbar label font=\footnotesize
}
\newganttchartelement{bpbar}{
  bpbar/.style={draw=none,fill=DarkGrey,shape=rounded rectangle,inner sep=0pt},
  %bpbar/.style={draw=none,fill=DarkGrey},
  bpbar label font=\footnotesize
}

\begin{ganttchart}[
    expand chart=1.5\textwidth,
    x unit=1mm,
    y unit title=5mm,
    y unit chart=5mm,
    %inline,
    canvas/.append style={fill=none,draw=none},
    title/.style={draw=none,fill=none},
    title height=1,
    title label font=\footnotesize,
    bar label font=\footnotesize,
    bar/.append style={draw=none,fill=Gold,rounded corners=3pt},
    milestone/.append style={fill=red,shape=diamond},
    milestone label font=\footnotesize,
    time slot format=isodate,
    %time slot unit=month,
    %link/.style={-latex, line width=1.5pt, linkred},
  ]{2032-12-01}{2035-02-28}
  \gantttitlecalendar{year,month} \\
  %\ganttbar[bar inline label node/.style=above]{Open detectors}{2033-01-01}{2033-01-15} 
  \ganttoutinbar[name=svc]{Remove and install services}{2032-12-01}{2033-12-31} \\
  \ganttbpbar[name=bpout]{Remove beam pipe (2 -- 4)}{2033-01-15}{2033-02-28} \\
  \ganttoutbar[name=sfout]{Remove SciFi and bridge}{2033-03-01}{2033-05-01} \\
  \ganttoutbar[name=r2out]{Remove RICH2}{2033-05-01}{2033-06-01} \\
  \ganttinbar[name=ms]{Install magnet stations}{2033-06-01}{2033-08-01} \\
  \ganttinbar[name=r2in]{Install RICH2/TORCH}{2033-07-01}{2034-04-01} \\
  \ganttinbar[name=brin]{Install bridge}{2033-08-01}{2033-10-01} \\
  \ganttinbar[name=mtin]{Install MT}{2033-10-01}{2034-04-01} 
  \ganttinbar[name=mtina]{}{2034-06-01}{2034-09-01} \\
  \ganttoutbar[name=calout]{Dismantle ECAL}{2033-03-01}{2033-07-01} \\
  \ganttbar[bar/.append style={shape=ellipse, fill=SkyBlue}]{Modify ECAL modules}{2033-04-15}{2034-02-01} \\
  \ganttinbar[name=calin]{Install PicoCal}{2033-10-01}{2034-04-01} \\
  \ganttoutinbar[name=mu]{Replace muon chambers}{2033-01-01}{2034-09-01} \\
  \ganttoutbar[name=utout]{Remove UT}{2033-01-01}{2033-03-01} \\
  \ganttbpbar[name=bp1out]{Remove RICH1 optics and beam pipe 1}{2033-03-01}{2033-04-01} \\
  \ganttoutbar[name=r1out]{Remove RICH1 mechanics}{2033-04-01}{2033-05-01} \\
  \ganttoutbar[name=veout]{Remove VELO}{2033-05-01}{2033-07-01} \\

  \ganttinbar[name=rfin]{Install VELO vessel}{2033-08-01}{2033-10-01} \\
  \ganttinbar[name=r1in1]{Install RICH1 mechanics}{2033-10-01}{2033-11-15} \\
  \ganttbpbar[name=bp1in]{Install beam pipe 1}{2033-11-15}{2033-12-01} \\
  \ganttinbar[name=utin]{Install UP}{2033-12-01}{2034-04-01} \\
  \ganttbpbar[name=bpin]{Install beam pipe (2 -- 4), bakeout}{2034-04-01}{2034-06-01} \\
  \ganttinbar[name=r1in2]{Install RICH1 optics and photon detectors}{2034-06-01}{2034-07-15} \\
  \ganttinbar[name=vein]{Install VELO modules}{2034-07-15}{2034-09-01} \\
  \ganttbar[name=co]{Global commissioning}{2034-09-01}{2035-03-01} 
  %\ganttbar[name=co1,inline=true,bar label inline node/.style=below]{$\neq$ margin for installation}{2034-09-01}{2035-03-01}
  %\ganttvrule[vrule/.append style={thin,dashed}]{}{2034-04-01}
\end{ganttchart}
\node[anchor=north east,font=\footnotesize] at (-1,0) {Baseline scenario};
\end{tikzpicture}


==> figs/LS4ScheduleFrugal.tex <==

\begin{tikzpicture}
\newganttchartelement{outbar}{
  outbar/.style={draw=none,fill=DarkGreen,shape=rounded rectangle,inner sep=0pt},
  outbar label font=\footnotesize
}
\newganttchartelement{inbar}{
  inbar/.style={draw=none,fill=DarkPlum,shape=rounded rectangle,inner sep=0pt},
  inbar label font=\footnotesize
}
\newganttchartelement{outinbar}{
  outinbar/.style={draw=none,left color=DarkGreen,right color=DarkPlum,shape=rounded rectangle,inner sep=0pt},
  outinbar label font=\footnotesize
}
\newganttchartelement{bpbar}{
  bpbar/.style={draw=none,fill=DarkGrey,shape=rounded rectangle,inner sep=0pt},
  %bpbar/.style={draw=none,fill=DarkGrey},
  bpbar label font=\footnotesize
}

\begin{ganttchart}[
    expand chart=\textwidth,
    x unit=0.1cm,
    y unit title=3.5mm,
    y unit chart=3.5mm,
    %inline,
    canvas/.append style={fill=none,draw=none},
    title/.style={draw=none,fill=none},
    title height=1,
    title label font=\footnotesize,
    bar label font=\footnotesize,
    bar/.append style={draw=none,fill=Gold,rounded corners=3pt},
    milestone/.append style={fill=red,shape=diamond},
    milestone label font=\footnotesize,
    time slot format=isodate,
    %time slot unit=month,
    %link/.style={-latex, line width=1.5pt, linkred},
  ]{2032-12-01}{2035-02-28}
  \gantttitlecalendar{year,month} \\
  %\ganttbar[bar inline label node/.style=above]{Open detectors}{2033-01-01}{2033-01-15} 
  \ganttoutinbar[name=svc]{Remove and install services}{2032-12-01}{2033-12-31} \\
  \ganttbpbar[name=bpout]{Remove beam pipe (2 -- 4)}{2033-01-15}{2033-02-28} \\
  \ganttoutbar[name=sfout]{Remove SciFi and bridge}{2033-03-01}{2033-05-01} \\
  \ganttoutinbar[name=r2]{Upgrade RICH2 in situ}{2033-05-01}{2034-04-01} \\
  \ganttinbar[name=brin]{Install bridge}{2033-07-01}{2033-09-01} \\
  \ganttinbar[name=mtin]{Install MT}{2033-09-01}{2034-04-01} 
  \ganttinbar[name=mtina]{}{2034-06-01}{2034-09-01} \\
  \ganttoutbar[name=calout]{Dismantle ECAL}{2033-03-01}{2033-07-01} \\
  \ganttbar[bar/.append style={shape=ellipse, fill=SkyBlue}]{Modify ECAL modules}{2033-04-15}{2034-02-01} \\
  \ganttinbar[name=calin]{Install PicoCal}{2033-10-01}{2034-04-01} \\
  \ganttoutinbar[name=mu]{Replace muon chambers}{2033-01-01}{2034-09-01} \\
  \ganttoutbar[name=utout]{Remove UT}{2033-01-01}{2033-03-01} \\
  \ganttbpbar[name=bp1out]{Remove RICH1 optics and beam pipe 1}{2033-03-01}{2033-04-01} \\
  \ganttoutbar[name=r1out]{Remove RICH1 mechanics}{2033-04-01}{2033-05-01} \\
  \ganttoutbar[name=veout]{Remove VELO}{2033-05-01}{2033-07-01} \\

  \ganttinbar[name=rfin]{Install VELO vessel}{2033-08-01}{2033-10-01} \\
  \ganttinbar[name=r1in1]{Install RICH1 mechanics}{2033-10-01}{2033-11-15} \\
  \ganttbpbar[name=bp1in]{Install beam pipe 1}{2033-11-15}{2033-12-01} \\
  \ganttinbar[name=utin]{Install UT}{2033-12-01}{2034-04-01} \\
  \ganttbpbar[name=bpin]{Install beam pipe (2 -- 4), bakeout}{2034-04-01}{2034-06-01} \\
  \ganttinbar[name=r1in2]{Install RICH1 optics and photon detectors}{2034-06-01}{2034-07-15} \\
  \ganttinbar[name=vein]{Install VELO modules}{2034-07-15}{2034-09-01} \\
  \ganttbar[name=co]{Global commissioning}{2034-09-01}{2035-03-01} 
  %\ganttbar[name=co1,inline=true,bar label inline node/.style=below]{$\neq$ margin for installation}{2034-09-01}{2035-03-01}
  %\ganttvrule[vrule/.append style={thin,dashed}]{}{2034-04-01}
  %\ganttmilestone{Start of commissioning}{2034-09-01}
\end{ganttchart}
\node[anchor=north east,font=\footnotesize] at (-1,0) {Frugal scenario};
\end{tikzpicture}


==> summary.tex <==
\section{Summary}
\label{sec:Summary}

A second major upgrade of the LHCb detector is necessary to maximise the physics potential of the HL-LHC.  
It will be installed after the completion of Run~4, by when the current detector will have accumulated its design integrated luminosity of $50 \invfb$. 
As shown in the LHCb \upgradetwo framework TDR~\cite{LHCb-TDR-023}, by equipping subdetectors to provide fast timing information and using radiation-hard technologies, it will be possible to operate at instantaneous luminosity of up to $1.5 \times 10^{34} \cm^{-2}\sec^{-1}$ while maintaining or even exceeding the detector performance in the current experiment.
This will enable a total sample exceeding $300 \invfb$ to be integrated by the end of HL-LHC operation, and will give unprecedented sensitivity to physics beyond the Standard Model in beauty and charm physics.
LHCb \upgradetwo\ will additionally provide several other unique science opportunities, including in hadron spectroscopy, in electroweak precision measurements, in dark sector searches and in studies of heavy ion collisions. 
The European Strategy for Particle Physics vision of full exploitation of the High Luminosity LHC (HL-LHC), including flavour physics, can only be achieved with LHCb \upgradetwo.

Since the approval of the framework TDR, significant progress has been made towards the design of an experiment that can be constructed and installed in the available time frame.
Further studies in collaboration with the LHC accelerator division have confirmed that  LHCb \upgradetwo will not significantly impact on ATLAS and CMS operation during the HL-LHC era.
Additionally, a flat optics configuration has been developed, which can provide higher integrated luminosity in the LHCb interaction region.  
Although not yet validated with dynamic aperature studies and dedicated machine tests, this provides a very promising scenario and illustrates robustness in the expected accelerator performance.

On the detector side, a re-evaluation of the baseline choices made in the framework TDR has been carried out in light of ongoing R\&D activities.  
As a result, the FTDR design is largely confirmed.
A reduction of the fraction of the Mighty Tracker area using silicon pixels is achieved thanks to improvement in the scintillating fibre technology that covers the remaining area.
The area covered by the Upstream Pixel tracker is also reduced, removing outer regions where hits are not required to reconstruct good quality long tracks. 
The design of the PicoCal is updated to re-use, after refurbishment, modules from the present electromagnetic calorimeter in the outermost regions where the requirements allow this.
The cost reduction from these optimisations is compensated by an increase in other subdetectors due to a combination of inflation-related effects and design updates. 
The total Baseline scenario cost is $\sim 182$\,MCHF, which exceeds only slightly the value estimated in the framework TDR. 

In addition to re-evaluation of the Baseline scenario, detector scoping options have been explored, with the aim of establishing scenarios at reduced cost and complexity of the overall project.
Two descoped scenarios, Middle and Low, have been identified with cost envelopes estimated at $\sim 156$\,MCHF and $\sim 125$\,MCHF, respectively. 
In both cases the peak luminosity is reduced from 1.5 to $1.0 \times 10^{34}\cm^{-2}\sec^{-1}$. 
Due to the longer levelling time at lower peak luminosity, the reduction in total LHCb integrated luminosity is proportionately less than that of the peak value, but is still significant at $\sim 12$\% (or $\sim 20$\% with flat optics). 
However, the corresponding decreases of peak detector occupancy and data throughput lead to important simplifications in the detector design, with associated cost savings.
Additionally, the longer levelling time will provide operational stability, which is expected to be important for the high precision measurements at the core of the physics programme. 

In the Middle scenario, the area covered by silicon pixels in the Mighty Tracker is further reduced from the Baseline configuration, and significantly less investment is required in the trigger farm. 
Both the Muon and RICH detectors have reduced granularity, and the active area of the TORCH detector is reduced.
Additional shielding before the Muon stations is not required, reducing the complexity of the infrastructure requirements.

In the Low scenario, the TORCH detector and the Magnet Stations are eliminated, reducing the overall complexity of the project but at significant loss in physics capability. 
The active areas of both the Upstream Pixel tracker and the Mighty Tracker scintillating fibres are reduced, and some VELO stations are removed, with a direct impact on acceptance.
A more conservative VELO module substrate with increased material is used, with equally direct consequences for the impact parameter resolution, which is crucial for the efficient operation of LHCb's real time analysis system.
Single rather than double readout is used in the outer region of the PicoCal, and the RICH2 optical system and its vessel are not upgraded.  
The cost of the trigger farm is further reduced, which may necessitate a narrowing of the physics programme if it is not possible to process all channels of interest with the available resources.

The impact of the different scenarios on physics performance has been studied.
The Middle scenario has less redundancy than the Baseline, with the reduction in capability of operating at the highest pile-up reducing the flexibility to compensate for possible changes in the LHC operation such as the number of colliding bunches in LHCb or the number of physics days.  
Nonetheless, this scenario is still expected to provide robust tracking and PID performance, since the reduction of granularity is balanced by the reduction of peak luminosity.
The lower integrated luminosity will reduce the achievable sensitivity across the physics programme.
On the other hand, the longer levelling time operating at instantaneous luminosity of $1.0 \times 10^{34}\cm^{-2}\sec^{-1}$ will have some advantages for stable operation of the detector.
%Indeed, in some cases the performance at instantaneous luminosity of $1.0 \times 10^{34}\cm^{-2}\sec^{-1}$ in the Middle scenario is superior to that at $1.5 \times 10^{34}\cm^{-2}\sec^{-1}$ in the Baseline scenario.
%
In the Low scenario, the loss of redundancy in detector features puts at risk the success of some key measurements that require the full detector capabilities.
A good programme of measurements is expected to still be possible, but is likely to be less broad in scope.
It will also be challenging to achieve the highly precise measurements that are planned due to worse signal-background separation and increased detector material.

Plans for the project organisation and schedule have also been developed since the framework TDR.  
The proposed organisation is based on experience from previous construction projects, both for LHCb and other experiments.
Technical Design Reports for the subdetectors are anticipated in 2026, after which the project will move to the construction phase.  
Each subdetector has developed a plan to complete construction by mid-2032, so that installation can proceed during the two years of Long Shutdown 4 currently scheduled for 2033--34, and be ready for data-taking at the start of Run~5 in 2035. 
The required human resources and technical infrastructure have also been scrutinised.
The main risks associated with these schedules have been identified and work is already ongoing to prepare mitigation plans. 

To conclude, three detector scenarios, Baseline, Middle and Low, have been considered.
These correspond to different cost ranges, and also have implications for the overall complexity of the project and the required human resources and technical infrastructure.
Each can be considered plausible depending on assumptions on the support from Funding Agencies and the growth of the collaboration.  
An exciting and unique physics programme will be possible in each scenario, although the reduction of integrated luminosity and detector features in the downscoped scenarios has a clear impact on the anticipated physics performance.
The higher cost of the Baseline and (to some extent) Middle scenarios not only results in improved performance and a stronger science programme, but also provides additional robustness to achieve the goal of full exploitation of the HL-LHC.

